Basic Notions for the Analysis of Large Affiliation Networks / Bipartite Graphs

Many real-world complex networks actually have a bipartite nature: their nodes may be separated into two classes, the links being between nodes of different classes only. Despite this, and despite the fact that many ad-hoc tools have been designed for the study of special cases, very few exist to analyse (describe, extract relevant information) such networks in a systematic way. We propose here an extension of the most basic notions used nowadays to analyse classical complex networks to the bipartite case. To achieve this, we introduce a set of simple statistics, which we discuss by comparing their values on a representative set of real-world networks and on their random versions.

==> Plots/actor/bot/bot_n.tex <==
127\mbox{,}823

==> Plots/actor/bot/cc_vee.tex <==
0.0082

==> Plots/actor/bot/classical_avg_dist.tex <==
7.2

==> Plots/actor/bot/classical_delta.tex <==
0.000011

==> Plots/actor/bot/classical_k.tex <==
5.7

==> Plots/actor/bot/classical_m.tex <==
1\mbox{,}470\mbox{,}418

==> Plots/actor/bot/classical_n.tex <==
511\mbox{,}463

==> Plots/actor/bot/classical_size_giant.tex <==
498\mbox{,}925

==> Plots/actor/bot/delta.tex <==
0.000030

==> Plots/actor/bot/k_bot.tex <==
11.5

==> Plots/actor/bot/k_top.tex <==
3.8

==> Plots/actor/bot/nb_N.tex <==
849\mbox{,}460\mbox{,}634

==> Plots/actor/bot/nb_bow.tex <==
3\mbox{,}503\mbox{,}277

==> Plots/actor/bot/proj_avg_dist.tex <==
3.7

==> Plots/actor/bot/proj_delta.tex <==
0.00020

==> Plots/actor/bot/proj_k.tex <==
78.4

==> Plots/actor/bot/proj_n.tex <==
383\mbox{,}640

==> Plots/actor/bot/proj_size_giant.tex <==
374\mbox{,}511

==> Plots/actor/bot/top_n.tex <==
383\mbox{,}640

==> Plots/actor/random/bot/bot_n.tex <==
127\mbox{,}823

==> Plots/actor/random/bot/cc_vee.tex <==
0.00024

==> Plots/actor/random/bot/classical_avg_dist.tex <==
5.8

==> Plots/actor/random/bot/classical_delta.tex <==
0.000011

==> Plots/actor/random/bot/classical_k.tex <==
5.7

==> Plots/actor/random/bot/classical_m.tex <==
1\mbox{,}470\mbox{,}039

==> Plots/actor/random/bot/classical_n.tex <==
511\mbox{,}463

==> Plots/actor/random/bot/classical_size_giant.tex <==
507\mbox{,}375

==> Plots/actor/random/bot/delta.tex <==
0.000030

==> Plots/actor/random/bot/k_bot.tex <==
11.5

==> Plots/actor/random/bot/k_top.tex <==
3.8

==> Plots/actor/random/bot/m.tex <==
1\mbox{,}470\mbox{,}039

==> Plots/actor/random/bot/nb_N.tex <==
1\mbox{,}030\mbox{,}012\mbox{,}266

==> Plots/actor/random/bot/nb_bow.tex <==
122\mbox{,}897

==> Plots/actor/random/bot/proj_avg_dist.tex <==
3.0

==> Plots/actor/random/bot/proj_delta.tex <==
0.00022

==> Plots/actor/random/bot/proj_k.tex <==
85.6

==> Plots/actor/random/bot/proj_m.tex <==
16\mbox{,}426\mbox{,}643

==> Plots/actor/random/bot/proj_n.tex <==
383\mbox{,}640

==> Plots/actor/random/bot/proj_size_giant.tex <==
381\mbox{,}431

==> Plots/actor/random/bot/top_n.tex <==
383\mbox{,}640

==> Plots/actor/random/top/bot_n.tex <==
383\mbox{,}640

==> Plots/actor/random/top/classical_delta.tex <==
0.000011

==> Plots/actor/random/top/classical_k.tex <==
5.7

==> Plots/actor/random/top/classical_m.tex <==
1\mbox{,}470\mbox{,}039

==> Plots/actor/random/top/classical_n.tex <==
511\mbox{,}463

==> Plots/actor/random/top/classical_size_giant.tex <==
507\mbox{,}375

==> Plots/actor/random/top/delta.tex <==
0.000030

==> Plots/actor/random/top/k_bot.tex <==
3.8

==> Plots/actor/random/top/k_top.tex <==
11.5

==> Plots/actor/random/top/m.tex <==
1\mbox{,}470\mbox{,}039

==> Plots/actor/random/top/nb_N.tex <==
1\mbox{,}030\mbox{,}012\mbox{,}266

==> Plots/actor/random/top/nb_bow.tex <==
122\mbox{,}897

==> Plots/actor/random/top/proj_avg_dist.tex <==
2.5

==> Plots/actor/random/top/proj_delta.tex <==
0.0028

==> Plots/actor/random/top/proj_k.tex <==
356.3

==> Plots/actor/random/top/proj_m.tex <==
22\mbox{,}768\mbox{,}907

==> Plots/actor/random/top/proj_n.tex <==
127\mbox{,}823

==> Plots/actor/random/top/proj_size_giant.tex <==
125\mbox{,}944

==> Plots/actor/random/top/top_n.tex <==
127\mbox{,}823

==> Plots/actor/top/classical_delta.tex <==
0.000011

==> Plots/actor/top/classical_m.tex <==
1\mbox{,}470\mbox{,}418

==> Plots/actor/top/classical_n.tex <==
511\mbox{,}463

==> Plots/actor/top/classical_size_giant.tex <==
498\mbox{,}925

==> Plots/actor/top/nb_N.tex <==
849\mbox{,}459\mbox{,}918

==> Plots/actor/top/nb_bow.tex <==
3\mbox{,}503\mbox{,}289

==> Plots/actor/top/proj_avg_dist.tex <==
3.1

==> Plots/actor/top/proj_delta.tex <==
0.0025

==> Plots/actor/top/proj_k.tex <==
320.6

==> Plots/actor/top/proj_n.tex <==
127\mbox{,}823

==> Plots/actor/top/proj_size_giant.tex <==
124\mbox{,}414

==> Plots/coauthoring/bot/bot_n.tex <==
19\mbox{,}885

==> Plots/coauthoring/bot/cc_vee.tex <==
0.079

==> Plots/coauthoring/bot/classical_avg_dist.tex <==
13.3

==> Plots/coauthoring/bot/classical_delta.tex <==
0.000070

==> Plots/coauthoring/bot/classical_k.tex <==
2.5

==> Plots/coauthoring/bot/classical_m.tex <==
45\mbox{,}904

==> Plots/coauthoring/bot/classical_n.tex <==
36\mbox{,}285

==> Plots/coauthoring/bot/classical_size_giant.tex <==
27\mbox{,}863

==> Plots/coauthoring/bot/delta.tex <==
0.00014

==> Plots/coauthoring/bot/k_bot.tex <==
2.3

==> Plots/coauthoring/bot/k_top.tex <==
2.8

==> Plots/coauthoring/bot/m.tex <==
45\mbox{,}904

==> Plots/coauthoring/bot/nb_N.tex <==
541\mbox{,}227

==> Plots/coauthoring/bot/nb_bow.tex <==
21\mbox{,}310

==> Plots/coauthoring/bot/proj_avg_dist.tex <==
7.2

==> Plots/coauthoring/bot/proj_delta.tex <==
0.00022

==> Plots/coauthoring/bot/proj_k.tex <==
3.6

==> Plots/coauthoring/bot/proj_n.tex <==
16\mbox{,}400

==> Plots/coauthoring/bot/proj_size_giant.tex <==
11\mbox{,}654

==> Plots/coauthoring/bot/top_n.tex <==
16\mbox{,}400

==> Plots/coauthoring/random/bot/bot_n.tex <==
19\mbox{,}885

==> Plots/coauthoring/random/bot/cc_vee.tex <==
0.00012

==> Plots/coauthoring/random/bot/classical_avg_dist.tex <==
9.5

==> Plots/coauthoring/random/bot/classical_delta.tex <==
0.000070

==> Plots/coauthoring/random/bot/classical_k.tex <==
2.5

==> Plots/coauthoring/random/bot/classical_m.tex <==
45\mbox{,}895

==> Plots/coauthoring/random/bot/classical_n.tex <==
36\mbox{,}285

==> Plots/coauthoring/random/bot/classical_size_giant.tex <==
33\mbox{,}119

==> Plots/coauthoring/random/bot/delta.tex <==
0.00014

==> Plots/coauthoring/random/bot/k_bot.tex <==
2.3

==> Plots/coauthoring/random/bot/k_top.tex <==
2.8

==> Plots/coauthoring/random/bot/m.tex <==
45\mbox{,}895

==> Plots/coauthoring/random/bot/nb_N.tex <==
532\mbox{,}247

==> Plots/coauthoring/random/bot/nb_bow.tex <==
33

==> Plots/coauthoring/random/bot/proj_avg_dist.tex <==
5.0

==> Plots/coauthoring/random/bot/proj_delta.tex <==
0.00030

==> Plots/coauthoring/random/bot/proj_k.tex <==
4.9

==> Plots/coauthoring/random/bot/proj_m.tex <==
39\mbox{,}960

==> Plots/coauthoring/random/bot/proj_n.tex <==
16\mbox{,}400

==> Plots/coauthoring/random/bot/proj_size_giant.tex <==
14\mbox{,}607

==> Plots/coauthoring/random/bot/top_n.tex <==
16\mbox{,}400

==> Plots/coauthoring/random/top/bot_n.tex <==
16\mbox{,}400

==> Plots/coauthoring/random/top/classical_delta.tex <==
0.000070

==> Plots/coauthoring/random/top/classical_k.tex <==
2.5

==> Plots/coauthoring/random/top/classical_m.tex <==
45\mbox{,}895

==> Plots/coauthoring/random/top/classical_n.tex <==
36\mbox{,}285

==> Plots/coauthoring/random/top/classical_size_giant.tex <==
33\mbox{,}119

==> Plots/coauthoring/random/top/delta.tex <==
0.00014

==> Plots/coauthoring/random/top/k_bot.tex <==
2.8

==> Plots/coauthoring/random/top/k_top.tex <==
2.3

==> Plots/coauthoring/random/top/m.tex <==
45\mbox{,}895

==> Plots/coauthoring/random/top/nb_N.tex <==
532\mbox{,}247

==> Plots/coauthoring/random/top/nb_bow.tex <==
33

==> Plots/coauthoring/random/top/proj_avg_dist.tex <==
4.5

==> Plots/coauthoring/random/top/proj_delta.tex <==
0.00077

==> Plots/coauthoring/random/top/proj_k.tex <==
15.4

==> Plots/coauthoring/random/top/proj_m.tex <==
152\mbox{,}945

==> Plots/coauthoring/random/top/proj_n.tex <==
19\mbox{,}885

==> Plots/coauthoring/random/top/proj_size_giant.tex <==
18\mbox{,}512

==> Plots/coauthoring/random/top/top_n.tex <==
19\mbox{,}885

==> Plots/coauthoring/top/classical_delta.tex <==
0.000070

==> Plots/coauthoring/top/classical_m.tex <==
45\mbox{,}904

==> Plots/coauthoring/top/classical_n.tex <==
36\mbox{,}285

==> Plots/coauthoring/top/classical_size_giant.tex <==
27\mbox{,}863

==> Plots/coauthoring/top/nb_N.tex <==
541\mbox{,}135

==> Plots/coauthoring/top/nb_bow.tex <==
21\mbox{,}313

==> Plots/coauthoring/top/proj_avg_dist.tex <==
6.4

==> Plots/coauthoring/top/proj_delta.tex <==
0.00068

==> Plots/coauthoring/top/proj_k.tex <==
13.5

==> Plots/coauthoring/top/proj_n.tex <==
19\mbox{,}885

==> Plots/coauthoring/top/proj_size_giant.tex <==
16\mbox{,}209

==> Plots/cooccurrence/bot/bot_n.tex <==
13\mbox{,}587

==> Plots/cooccurrence/bot/cc_vee.tex <==
0.043

==> Plots/cooccurrence/bot/classical_avg_dist.tex <==
3.3

==> Plots/cooccurrence/bot/classical_delta.tex <==
0.00070

==> Plots/cooccurrence/bot/classical_k.tex <==
16.0

==> Plots/cooccurrence/bot/classical_m.tex <==
183\mbox{,}363

==> Plots/cooccurrence/bot/classical_n.tex <==
22\mbox{,}851

==> Plots/cooccurrence/bot/classical_size_giant.tex <==
22\mbox{,}825

==> Plots/cooccurrence/bot/delta.tex <==
0.0015

==> Plots/cooccurrence/bot/k_bot.tex <==
13.5

==> Plots/cooccurrence/bot/k_top.tex <==
19.8

==> Plots/cooccurrence/bot/m.tex <==
183\mbox{,}363

==> Plots/cooccurrence/bot/nb_N.tex <==
-\mbox{,}895\mbox{,}776\mbox{,}829

==> Plots/cooccurrence/bot/nb_bow.tex <==
73\mbox{,}094\mbox{,}403

==> Plots/cooccurrence/bot/proj_avg_dist.tex <==
2.1

==> Plots/cooccurrence/bot/proj_delta.tex <==
0.0091

==> Plots/cooccurrence/bot/proj_k.tex <==
84.6

==> Plots/cooccurrence/bot/proj_n.tex <==
9\mbox{,}264

==> Plots/cooccurrence/bot/proj_size_giant.tex <==
9\mbox{,}246

==> Plots/cooccurrence/bot/top_n.tex <==
9\mbox{,}264

==> Plots/cooccurrence/random/bot/bot_n.tex <==
13\mbox{,}587

==> Plots/cooccurrence/random/bot/cc_vee.tex <==
0.048

==> Plots/cooccurrence/random/bot/classical_avg_dist.tex <==
3.3

==> Plots/cooccurrence/random/bot/classical_delta.tex <==
0.00066

==> Plots/cooccurrence/random/bot/classical_k.tex <==
15.0

==> Plots/cooccurrence/random/bot/classical_m.tex <==
171\mbox{,}368

==> Plots/cooccurrence/random/bot/classical_n.tex <==
22\mbox{,}851

==> Plots/cooccurrence/random/bot/classical_size_giant.tex <==
22\mbox{,}851

==> Plots/cooccurrence/random/bot/delta.tex <==
0.0014

==> Plots/cooccurrence/random/bot/k_bot.tex <==
12.6

==> Plots/cooccurrence/random/bot/k_top.tex <==
18.5

==> Plots/cooccurrence/random/bot/m.tex <==
171\mbox{,}368

==> Plots/cooccurrence/random/bot/nb_N.tex <==
-1\mbox{,}497\mbox{,}917\mbox{,}616

==> Plots/cooccurrence/random/bot/nb_bow.tex <==
66\mbox{,}797\mbox{,}316

==> Plots/cooccurrence/random/bot/proj_avg_dist.tex <==
2.0

==> Plots/cooccurrence/random/bot/proj_delta.tex <==
0.011

==> Plots/cooccurrence/random/bot/proj_k.tex <==
104.2

==> Plots/cooccurrence/random/bot/proj_m.tex <==
482\mbox{,}633

==> Plots/cooccurrence/random/bot/proj_n.tex <==
9\mbox{,}264

==> Plots/cooccurrence/random/bot/proj_size_giant.tex <==
9\mbox{,}264

==> Plots/cooccurrence/random/bot/top_n.tex <==
9\mbox{,}264

==> Plots/cooccurrence/random/top/bot_n.tex <==
9\mbox{,}264

==> Plots/cooccurrence/random/top/classical_delta.tex <==
0.00066

==> Plots/cooccurrence/random/top/classical_k.tex <==
15.0

==> Plots/cooccurrence/random/top/classical_m.tex <==
171\mbox{,}368

==> Plots/cooccurrence/random/top/classical_n.tex <==
22\mbox{,}851

==> Plots/cooccurrence/random/top/classical_size_giant.tex <==
22\mbox{,}851

==> Plots/cooccurrence/random/top/delta.tex <==
0.0014

==> Plots/cooccurrence/random/top/k_bot.tex <==
18.5

==> Plots/cooccurrence/random/top/k_top.tex <==
12.6

==> Plots/cooccurrence/random/top/m.tex <==
171\mbox{,}368

==> Plots/cooccurrence/random/top/nb_N.tex <==
-1\mbox{,}497\mbox{,}917\mbox{,}616

==> Plots/cooccurrence/random/top/nb_bow.tex <==
66\mbox{,}797\mbox{,}316

==> Plots/cooccurrence/random/top/proj_avg_dist.tex <==
1.4

==> Plots/cooccurrence/random/top/proj_delta.tex <==
0.61

==> Plots/cooccurrence/random/top/proj_k.tex <==
8278.2

==> Plots/cooccurrence/random/top/proj_m.tex <==
56\mbox{,}237\mbox{,}778

==> Plots/cooccurrence/random/top/proj_n.tex <==
13\mbox{,}587

==> Plots/cooccurrence/random/top/proj_size_giant.tex <==
13\mbox{,}587

==> Plots/cooccurrence/random/top/top_n.tex <==
13\mbox{,}587

==> Plots/cooccurrence/top/classical_delta.tex <==
0.00070

==> Plots/cooccurrence/top/classical_m.tex <==
183\mbox{,}363

==> Plots/cooccurrence/top/classical_n.tex <==
22\mbox{,}851

==> Plots/cooccurrence/top/classical_size_giant.tex <==
22\mbox{,}825

==> Plots/cooccurrence/top/nb_N.tex <==
-1\mbox{,}191\mbox{,}031\mbox{,}716

==> Plots/cooccurrence/top/nb_bow.tex <==
81\mbox{,}910\mbox{,}875

==> Plots/cooccurrence/top/proj_avg_dist.tex <==
1.4

==> Plots/cooccurrence/top/proj_delta.tex <==
0.56

==> Plots/cooccurrence/top/proj_k.tex <==
7566.8

==> Plots/cooccurrence/top/proj_n.tex <==
13\mbox{,}587

==> Plots/cooccurrence/top/proj_size_giant.tex <==
13\mbox{,}579

==> Plots/p2p/bot/bot_n.tex <==
1\mbox{,}986\mbox{,}588

==> Plots/p2p/bot/cc_vee.tex <==
0.0094

==> Plots/p2p/bot/classical_avg_dist.tex <==
5.3

==> Plots/p2p/bot/classical_delta.tex <==
0.0000021

==> Plots/p2p/bot/classical_k.tex <==
15.2

==> Plots/p2p/bot/classical_m.tex <==
55\mbox{,}829\mbox{,}392

==> Plots/p2p/bot/classical_n.tex <==
7\mbox{,}367\mbox{,}134

==> Plots/p2p/bot/classical_size_giant.tex <==
7\mbox{,}366\mbox{,}850

==> Plots/p2p/bot/delta.tex <==
0.0000052

==> Plots/p2p/bot/k_bot.tex <==
28.1

==> Plots/p2p/bot/k_top.tex <==
10.4

==> Plots/p2p/bot/m.tex <==
55\mbox{,}829\mbox{,}392

==> Plots/p2p/bot/nb_N.tex <==
810\mbox{,}504\mbox{,}674\mbox{,}176


==> Plots/p2p/bot/nb_bow.tex <==
3\mbox{,}804\mbox{,}659\mbox{,}243


==> Plots/p2p/bot/proj_delta.tex <==
0.00070

==> Plots/p2p/bot/proj_k.tex <==
3770.2

==> Plots/p2p/bot/proj_n.tex <==
5\mbox{,}380\mbox{,}546

==> Plots/p2p/bot/top_n.tex <==
5\mbox{,}380\mbox{,}546

==> Plots/p2p/random/bot/bot_n.tex <==
1\mbox{,}427\mbox{,}284

==> Plots/p2p/random/bot/cc_vee.tex <==
0.00019

==> Plots/p2p/random/bot/classical_avg_dist.tex <==
5.0

==> Plots/p2p/random/bot/classical_delta.tex <==
0.0000019

==> Plots/p2p/random/bot/classical_k.tex <==
12.4

==> Plots/p2p/random/bot/classical_m.tex <==
40\mbox{,}161\mbox{,}121

==> Plots/p2p/random/bot/classical_n.tex <==
6\mbox{,}482\mbox{,}553

==> Plots/p2p/random/bot/classical_size_giant.tex <==
6\mbox{,}481\mbox{,}667

==> Plots/p2p/random/bot/delta.tex <==
0.0000056

==> Plots/p2p/random/bot/k_bot.tex <==
28.1

==> Plots/p2p/random/bot/k_top.tex <==
7.9

==> Plots/p2p/random/bot/m.tex <==
40\mbox{,}161\mbox{,}121

==> Plots/p2p/random/bot/nb_N.tex <==
606\mbox{,}814\mbox{,}644\mbox{,}945


==> Plots/p2p/random/bot/nb_bow.tex <==
56\mbox{,}321\mbox{,}865

==> Plots/p2p/random/bot/proj_delta.tex <==
0.00067

==> Plots/p2p/random/bot/proj_k.tex <==
3398.2

==> Plots/p2p/random/bot/proj_m.tex <==
8\mbox{,}589\mbox{,}528\mbox{,}173


==> Plots/p2p/random/bot/proj_n.tex <==
5\mbox{,}055\mbox{,}269

==> Plots/p2p/random/bot/top_n.tex <==
5\mbox{,}055\mbox{,}269

==> Plots/p2p/random/top/bot_n.tex <==
5\mbox{,}055\mbox{,}269

==> Plots/p2p/random/top/classical_delta.tex <==
0.0000019

==> Plots/p2p/random/top/classical_k.tex <==
12.4

==> Plots/p2p/random/top/classical_m.tex <==
40\mbox{,}161\mbox{,}121

==> Plots/p2p/random/top/classical_n.tex <==
6\mbox{,}482\mbox{,}553

==> Plots/p2p/random/top/classical_size_giant.tex <==
6\mbox{,}481\mbox{,}667

==> Plots/p2p/random/top/delta.tex <==
0.0000056

==> Plots/p2p/random/top/k_bot.tex <==
7.9

==> Plots/p2p/random/top/k_top.tex <==
28.1

==> Plots/p2p/random/top/m.tex <==
40\mbox{,}161\mbox{,}121

==> Plots/p2p/random/top/nb_N.tex <==
606\mbox{,}814\mbox{,}644\mbox{,}945


==> Plots/p2p/random/top/nb_bow.tex <==
56\mbox{,}321\mbox{,}865

==> Plots/p2p/random/top/proj_delta.tex <==
0.00067

==> Plots/p2p/random/top/proj_k.tex <==
954.8

==> Plots/p2p/random/top/proj_m.tex <==
681\mbox{,}369\mbox{,}727

==> Plots/p2p/random/top/proj_n.tex <==
1\mbox{,}427\mbox{,}284

==> Plots/p2p/random/top/top_n.tex <==
1\mbox{,}427\mbox{,}284

==> Plots/p2p/top/classical_delta.tex <==
0.0000021

==> Plots/p2p/top/classical_m.tex <==
55\mbox{,}829\mbox{,}392

==> Plots/p2p/top/classical_n.tex <==
7\mbox{,}367\mbox{,}134

==> Plots/p2p/top/classical_size_giant.tex <==
7\mbox{,}366\mbox{,}850

==> Plots/p2p/top/nb_N.tex <==
810\mbox{,}504\mbox{,}674\mbox{,}176


==> Plots/p2p/top/nb_bow.tex <==
3\mbox{,}804\mbox{,}659\mbox{,}243


==> Plots/p2p/top/proj_delta.tex <==
0.00055

==> Plots/p2p/top/proj_k.tex <==
1092.5

==> Plots/p2p/top/proj_n.tex <==
1\mbox{,}986\mbox{,}588
